STEMM: Self-learning with Speech-text Manifold Mixup for Speech Translation

How to learn a better speech representation for end-to-end speech-to-text translation (ST) with limited labeled data? Existing techniques often attempt to transfer powerful machine translation (MT) capabilities to ST, but neglect the representation discrepancy across modalities. In this paper, we propose the Speech-TExt Manifold Mixup (STEMM) method to calibrate such discrepancy. Specifically, we mix up the representation sequences of different modalities, and take both unimodal speech sequences and multimodal mixed sequences as input to the translation model in parallel, and regularize their output predictions with a self-learning framework. Experiments on MuST-C speech translation benchmark and further analysis show that our method effectively alleviates the cross-modal representation discrepancy, and achieves significant improvements over a strong baseline on eight translation directions.

==> Figures/case.tex <==

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{case.pdf}
    \caption{A schematic illustration of the difference between the representation of the speech sequence and the text sequence. In our work, mixup sequence is designed to fill the gap between them.}
    \label{fig:case}
\end{figure}


==> Figures/mixup-teacher.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{mixup-teacher.pdf}
    \caption{BLEU scores and prediction uncertainty with difference mixup ratio $p^*$ during inference. The metrics are calculated on MuST-C En-De \texttt{tst-COMMON} set.}
    \label{fig:mixup-teacher}
\end{figure}


==> Sections/045_mixup_is_teacher.tex <==
\input{Figures/mixup-teacher}

\label{sec:why-mixup-teacher}
In Section \ref{sec:dokd}, we use mixup translation task with different mixup ratio as a dynamic teacher. Intuitively, as mixup ratio $p^*$ increases (more acoustic tokens and less textual tokens), the model will predict translations with less accuracy and confidence, which can be considered as a weaker teacher. To prove this hypothesis, we perform inference under different mixup ratio $p^*$ with our trained model. As shown in Figure \ref{fig:mixup-teacher}, as the mixup ratio $p^*$ increases, the BLEU score keeps decreasing, and the prediction uncertainty (average entropy of the predicted probability distribution of all target tokens) keeps increasing, which fits our assumptions. Note that we calculate BLEU scores with free-running mode, while calculate uncertainty with teacher-forcing mode.



==> Tables/ablation.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{cccc}
\toprule
\textbf{Dynamic} & \textbf{KD} & \textbf{XMM}  & \textbf{BLEU} \\
\midrule
\checkmark & \checkmark & \checkmark &  \textbf{28.7} \\
\texttimes & \checkmark & \checkmark &  28.5 \\
\texttimes & \checkmark & \texttimes &  28.1 \\
\texttimes & \texttimes & \checkmark &  27.9 \\
\texttimes & \texttimes & \texttimes &  27.4 \\
\bottomrule
\end{tabular}
\caption{BLEU scores on MuST-C En-De \texttt{tst-COMMON} set with different finetuning strategy.}
\label{tab:ablation}
\end{table}
